Decentralized Asset Custody Scheme with Security against Rational Adversary

Asset custody is a core financial service in which the custodian holds in-safekeeping assets on behalf of the client. Although traditional custody service is typically endorsed by centralized authorities, decentralized custody scheme has become technically feasible since the emergence of digital assets, and furthermore, it is greatly needed by new applications such as blockchain and DeFi (Decentralized Finance). In this work, we propose a framework of decentralized asset custody scheme that is able to support a large number of custodians and safely hold customer assets of multiple times the value of the total security deposit. The proposed custody scheme distributes custodians and assets into many custodian groups via combinatorial designs, where each group fully controls the assigned assets. Since every custodian group is small, the overhead cost is significantly reduced. The liveness is also improved because even a single alive group would be able to process transactions. The security of this custody scheme is guaranteed under the rational adversary model, such that any adversary corrupting a bounded fraction of custodians cannot move assets more than the security deposit paid. We further analyze the security and performance of our constructions from both theoretical and experimental sides and give explicit examples with concrete numbers and figures for a better understanding of our results.

==> Sections/Hardness.tex <==
\section{Hardness Results}\label{sec:hardness}

In this section, we consider the hardness issue of finding the best corrupting strategy, given a group assignment scheme and the number of corrupted nodes. In general, we show that such problem is NP-hard, in the following theorem.
\begin{theorem}\label{thm:hardness}
    Suppose $1\leq r \leq k$ are given constants, where $r = \lceil \mu k + \epsilon \rceil$. Let $|S| = n$, and $\mathcal{A}$ be a group assignment scheme such that $m = |\mathcal{A}|$ is within a polynomial size of $n$, and all groups in $\mathcal{A}$ have size $k$. Further, suppose an adversary controlling $r < s = \gamma n < n$ nodes. Then, when $1 \leq r < k$, it is NP-hard for the adversary to find the optimal attacking strategy and compute the value $\maxcorruptedgroupnumber$.
\end{theorem}
\begin{comment}
\begin{proof}[Sketch]
	To show the NP-hardness of the problem with $1 < r < k$, we consider the MAX $s$-VC problem. For the details on the reduction step, please refer to Appendix~\ref{app:proof-thm-hardness}.
	\qed
\end{proof}
\end{comment}

Theorem~\ref{thm:hardness} is proven in Appendix~\ref{app:proof-thm-hardness}. Generally, it is hard for the computationally bounded adversary to figure out the best attacking strategy. Nevertheless, there is a deterministic algorithm for the adversary to figure out a strategy which corrupts at least an average amount of groups. Let $\kappa(\gamma) := \Pr[\mathcal{H}(n, s, k) \geq r]$. Apparently, $\kappa(\gamma) m$ is the expected number of groups that the adversary can corrupt when the $\gamma n$ corrupted nodes are chosen uniformly at random. We have the following theorem:
\begin{theorem}\label{thm:better-than-average}
    Let $\kappa(\gamma)$ be defined as above. Suppose computing each binomial coefficient with size $n$ takes time no more than $T(n)$. Then there is a deterministic algorithm that gives an attacking strategy which corrupts at least $\kappa(\gamma) m$ groups, running in time $O\left(kmnT(n)\right)$.
\end{theorem}

The proof of the theorem is given in Appendix~\ref{app:proof-thm-better-than-average}.
\begin{comment}
\begin{proof}[Sketch]
	Specifically, we construct a deterministic algorithm running in $O\left(kmnT(n)\right)$ time (see Algorithm~\ref{alg:better-than-average}) and prove that the algorithm always return a corrupting strategy behaving no beneath the average. Specifically, in each step, we judge whether or not to corrupt a node conditioning on previous choices. We prove that after each step before the algorithm ends, the conditional expectation of the number of corrupted groups is no less than average given previous decisions, and as a result, the algorithm always returns a solution no worse than average. For the construction of the algorithm and full proof, please see Appendix~\ref{app:proof-thm-better-than-average}.
	\qed
\end{proof}
\end{comment}


==> Sections/Preliminaries.tex <==
%!TEX root = ../main.tex
\section{Preliminaries}\label{sec:preliminaries}

\begin{interposition}[Hypergeometric distribution and tail bound]
	A hypergeometric distribution $\mathcal{H}(N, K, n)$ is a discrete probability distribution with the following probability mass function:
	\[\Pr[\mathcal{H}(N, K, n) = k] = \frac{\binom{K}{k}\binom{N - K}{n - k}}{\binom{N}{n}}.\]
	
	$\mathcal{H}(N, K, n)$ draws the distribution of the number of items with a feature in $n$ draws without replacement, from totally $N$ items, $K$ of which with that feature. We are mostly interested in the tail bound of Hypergeometric distribution. 
	% Specifically, we have the following theorem, by~\cite{Hoeffding63,chvatal79}.
	\begin{lemma}[From~\cite{chvatal79}]
		Let $X \sim \mathcal{H}(N, K, n)$ and $p = K/N$, then:
		\begin{align*}
		&\Pr[X \leq (p - t)n] \leq \exp(-nD(p - t \| p)) \leq \exp(-2nt^2), \quad 0 < t < p \\
		&\Pr[X \geq (p + t)n] \leq \exp(-nD(p + t \| p)) \leq \exp(-2nt^2), \quad 0 < t < 1 - p
		\end{align*}
		where $D(\cdot \| \cdot)$ stands for the Kullback-Leibler divergence with two input real numbers in $(0, 1)$ naturally generalized to corresponding Bernoulli distributions, i.e.
		\[D(a \| b) := a\cdot\ln \left({a}/{b}\right) + (1 - a)\cdot\ln \big((1 - a)/(1 - b)\big),\quad a, b\in (0, 1)\].
	\end{lemma}
	
	For $0 < a < b < c < 1$, the naturally generalized Kullback-Leibler divergence satisfies
	\[D(a \| b) < D(a \| c),  D(c \| b) < D(c \| a), D(b \| a) < D(c \| a), D(b \| c) < D(a \| c).\]
\end{interposition}

%\paragraph{Hypergeometric distribution and tail bound.}
%
%A hypergeometric distribution $\mathcal{H}(N, K, n)$ is a discrete probability distribution with the following probability mass function:
%\[\Pr[\mathcal{H}(N, K, n) = k] = \frac{\binom{K}{k}\binom{N - K}{n - k}}{\binom{N}{n}}.\]
%
%Hypergeometric distribution draws the probability of getting $k$ items with a feature in $n$ draws without replacement, from totally $N$ items, $K$ of which with that feature. We are mostly interested in the tail bound of Hypergeometric distribution. 
%% Specifically, we have the following theorem, by~\cite{Hoeffding63,chvatal79}.
%\begin{lemma}[From~\cite{Hoeffding63,chvatal79}]
%	Let $X \sim \mathcal{H}(N, K, n)$ and $p = K/N$, then we have the following:
%	\begin{align*}
%	&\Pr[X \leq (p - t)n] \leq \exp(-nD(p - t \| p)) \leq \exp(-2nt^2), \quad 0 < t < p \\
%	&\Pr[X \geq (p + t)n] \leq \exp(-nD(p + t \| p)) \leq \exp(-2nt^2), \quad 0 < t < 1 - p
%	\end{align*}
%	where $D(\cdot \| \cdot)$ stands for the Kullback-Leibler divergence with input real numbers naturally generalized to probability distributions, i.e.
%	$D(a \| b) := a\cdot\ln \left({a}/{b}\right) + (1 - a)\cdot\ln \big((1 - a)/(1 - b)\big)$, for $a, b\in (0,1)$.
%\end{lemma}
%
%For $0 < a < b < c < 1$, the naturally generalized Kullback-Leibler divergence satisfies $D(a \| b) < D(a \| c)$,  $D(c \| b) < D(c \| a)$, $D(b \| a) < D(c \| a)$, $D(b \| c) < D(a \| c)$.

% We remark on the following important property of Kullback-Leibler divergence on two real numbers in $(0, 1)$:

% \begin{corollary}
%     When $0 < a < b < c < 1$, 
%     \begin{align*}
%         &D(a \| b) < D(a \| c), \quad D(c \| b) < D(c \| a);\\
%         &D(b \| a) < D(c \| a), \quad D(b \| c) < D(a \| c).
%     \end{align*}
% \end{corollary}

% Pinsker's theorem~\cite{Csiszar11} shows that $D(a \| b) \geq 2(a - b)^2$.

\begin{interposition}[Stirling's formula]
	Stirling's formula provides a good estimation of factorial terms. 
	Specifically, we will use the following version.
	\begin{lemma}[From~\cite{Robbins55}]
		For any integer $n \geq 1$, we have 
		$\sqrt{2\pi} \cdot e^{-n}\cdot n^{n + \frac{1}{2}} < n! < e^{1 - n}\cdot n^{n + \frac{1}{2}}$.
	\end{lemma}
\end{interposition}

%\paragraph{Stirling's formula.}
%
%Stirling's formula provides a good estimation of factorial terms. 
%Specifically, we will use the following version.
%\begin{lemma}[From~\cite{Robbins55}]
%	For any integer $n \geq 1$, we have 
%	$\sqrt{2\pi} \cdot e^{-n}\cdot n^{n + \frac{1}{2}} < n! < e^{1 - n}\cdot n^{n + \frac{1}{2}}$.
%\end{lemma}

\begin{interposition}[Block design]
	A block design is a particular combinatorial design consisting of a set of elements and a family of subsets (called blocks) whose arrangements satisfy generalized concepts of balance and symmetry.
	% Intuitively, block designs are those group assignment schemes with rather symmetric properties.
	
	\begin{definition}[Block design, from~\cite{Stinson07}, with notation revised]
		Let $n, k, \lambda$ and $t$ be positive integers such that $n > k \geq t$. 
		A block design $(T, \mathcal{B})$ is called an $t$-$(n, k, \lambda)$-design if $T$ is a set with $|T| = n$ and $\mathcal{B}$ is a family of $k$-element subsets of $T$ (called blocks), such that
		every $t$-element subset of $T$ is contained in exactly $\lambda$ blocks in $\mathcal{B}$.
		% and $\mathcal{A}$ satisfies the following:
		% \begin{itemize}
		%     % \item $|S| = n$;
		%     \item each block in $\mathcal{A}$ contains exactly $k$ points in $S$;
		%     \item every set of $r$ distinct elements in $S$ is contained in exactly $\lambda$ blocks.
		% \end{itemize}
	\end{definition}
	
	% In general, it is permitted for a block design to contain repeated blocks. However, in this work, we only focus on the case with $\lambda = 1$, which eliminates such a possibility.
	In this work we mainly consider designs with $\lambda = 1$, and hence $\mathcal{B}$ does not contain duplicate blocks.
	
	% We directly have the following corollaries.
	\begin{corollary}
		In a $t$-$(n, k, \lambda)$-design, the number of blocks is $m = \lambda \left. \binom{n}{t} \middle/ \binom{k}{t} \right.$.
	\end{corollary}
	\begin{corollary}
		Suppose $(T, \mathcal{B})$ is an $t$-$(n, k, \lambda)$-design. Then for any $1 \leq w \leq t$, $(T, \mathcal{B})$ is also a $w$-$(n, k, \lambda_w)$-design, for
		$\lambda_w = \lambda\cdot{\binom{n - w}{t - w}}/{\binom{k - w}{t - w}}$.
	\end{corollary}
	\begin{corollary}
		Suppose $(T, \mathcal{B})$ is an $t$-$(n, k, \lambda)$-design. Then for any $W \subseteq T$ with size $|W|=w \leq t$, $(T - W, \{B - W: W \subseteq B \in \mathcal{B}\})$ is a $(t - w)$-$(n - w, k - w, \lambda)$-design.
	\end{corollary}
	
	Furthermore, we remark that although non-trivial block designs exist universally by~\cite{Stinson07},
	only very few such designs are explicitly constructed.
\end{interposition}

%\paragraph{Block design.}
%
%A block design is a particular combinatorial design consisting of a set of elements and a family of subsets (called blocks) whose arrangements satisfy generalized concepts of balance and symmetry.
%% Intuitively, block designs are those group assignment schemes with rather symmetric properties.
%
%\begin{definition}[Block design, from~\cite{Stinson07}, with notation revised]
%	Let $n, k, \lambda$ and $t$ be positive integers such that $n > k \geq t$. 
%	A block design $(T, \mathcal{B})$ is called an $t$-$(n, k, \lambda)$-design if
%	$|T| = n$ and $\mathcal{B}$ is a family of $k$-element subsets of $T$ (called blocks), such that
%	every $r$-element subset of $T$ is contained in exactly $\lambda$ blocks in $\mathcal{B}$.
%	% and $\mathcal{A}$ satisfies the following:
%	% \begin{itemize}
%	%     % \item $|S| = n$;
%	%     \item each block in $\mathcal{A}$ contains exactly $k$ points in $S$;
%	%     \item every set of $r$ distinct elements in $S$ is contained in exactly $\lambda$ blocks.
%	% \end{itemize}
%\end{definition}
%
%% In general, it is permitted for a block design to contain repeated blocks. However, in this work, we only focus on the case with $\lambda = 1$, which eliminates such a possibility.
%In this work we mainly consider designs with $\lambda = 1$, and hence $\mathcal{B}$ does not contain duplicate blocks.
%
%% We directly have the following corollaries.
%\begin{corollary}
%	In an $t$-$(n, k, \lambda)$-design, the number of blocks is $m = \lambda \left. \binom{n}{t} \middle/ \binom{k}{t} \right.$.
%\end{corollary}
%\begin{corollary}
%	Suppose $(T, \mathcal{B})$ is an $t$-$(n, k, \lambda)$-design. Then for any $1 \leq w \leq t$, $(T, \mathcal{B})$ is also a $w$-$(n, k, \lambda_w)$-design, for
%	$\lambda_w = \lambda\cdot{\binom{n - w}{r - w}}/{\binom{k - w}{r - w}}$.
%\end{corollary}
%\begin{corollary}
%	Suppose $(T, \mathcal{B})$ is an $t$-$(n, k, \lambda)$-design. Then for any $W \subseteq T$ with size $|W|=w \leq r$, $(T - W, \{B - W: W \subseteq B \in \mathcal{B}\})$ is a $(t - w)$-$(n - w, k - w, \lambda)$-design.
%\end{corollary}
%
%Furthermore, we remark that although non-trivial block designs exist universally by~\cite{Stinson07},
%only very few such designs are explicitly constructed.

% The following theorem shows that non-trivial block designs universally exist. Nevertheless, there are only a few such designs that we currently know. 
% We even cannot construct any non-trivial block designs with $r \geq 7$.
% \begin{lemma}[\cite{Stinson07}]
%     For all positive integers $r, k$ and $n$ such that $r < k < n - r$, there exists a non-trivial $r$-$(n, k, \lambda)$-design for some positive integer $\lambda$.
% \end{lemma}
